ACECODER: Acing Coder RL via Automated Test-Case Synthesis

Most progress in recent coder models has been driven by supervised fine-tuning (SFT), while the potential of reinforcement learning (RL) remains largely unexplored, primarily due to the lack of reliable reward data/model in the code domain. In this paper, we address this challenge by leveraging automated large-scale test-case synthesis to enhance code model training. Specifically, we design a pipeline that generates extensive (question, test-cases) pairs from existing code data. Using these test cases, we construct preference pairs based on pass rates over sampled programs to train reward models with Bradley-Terry loss. It shows an average of 10-point improvement for Llama-3.1-8B-Ins and 5-point improvement for Qwen2.5-Coder-7B-Ins through best-of-32 sampling, making the 7B model on par with 236B DeepSeek-V2.5. Furthermore, we conduct reinforcement learning with both reward models and test-case pass rewards, leading to consistent improvements across HumanEval, MBPP, BigCodeBench, and LiveCodeBench (V4). Notably, we follow the R1-style training to start from Qwen2.5-Coder-base directly and show that our RL training can improve model on HumanEval-plus by over 25\% and MBPP-plus by 6\% for merely 80 optimization steps. We believe our results highlight the huge potential of reinforcement learning in coder models.

==> tables/main_result_template.tex <==
\begin{table*}[!tbh]
    \centering
    \caption{CodeRM's best-of-n results. We evaluated the model on MBPP, HumanEval (HE), BigCodeBench (BCB), and LiveCodeBench (LCB). Specifically, we have evaluated the Completion (C) and Instruct (I) splits of BCB for both Hard (H) and Full (F) versions, and also the plus version for MBPP and HE.}
    \label{tab:wide-table}
    \small
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{llccccccccc}
        \toprule
        \makecell{Policy Model} & 
        \makecell{Method} & 
        \makecell{BCB-C-F} & 
        \makecell{BCB-C-H} & 
        \makecell{BCB-I-F} &
        \makecell{BCB-I-H} &
        \makecell{HE} & 
        \makecell{HE+} & 
        \makecell{LCB} &
        \makecell{MBPP} & 
        \makecell{MBPP+} \\
        \midrule
        \multirow[c]{4}{*}{CodeLlama-Ins} & CodeRM & \bfseries 32.46 & \bfseries 9.46 & \bfseries 26.84 & \bfseries 5.41 & \bfseries 59.15 & \bfseries 51.22 & \bfseries 16.69 & \bfseries 61.11 & \bfseries 51.32 \\
        & average & 14.84 & 2.53 & 11.06 & 1.60 & 31.10 & 26.64 & 8.81 & 46.28 & 39.37 \\
        & greedy & 24.21 & 4.05 & 22.54 & 4.05 & 40.24 & 34.76 & 9.47 & 54.23 & 45.50 \\
        & oracle & 51.49 & 22.30 & 42.98 & 14.86 & 75.00 & 69.51 & 19.78 & 82.28 & 71.43 \\
        \midrule
        \multirow[c]{4}{*}{Llama-3.1-Ins} & CodeRM & \bfseries 43.51 & \bfseries 17.57 & \bfseries 34.39 & \bfseries 16.22 & \bfseries 73.17 & \bfseries 66.46 & \bfseries 25.67 & \bfseries 76.19 & \bfseries 63.23 \\
        & average & 31.09 & 8.83 & 25.87 & 9.04 & 61.43 & 54.19 & 13.83 & 64.70 & 54.81 \\
        & greedy & 38.51 & 12.84 & 31.84 & 13.51 & 68.90 & 62.20 & 17.99 & 67.20 & 54.76 \\
        & oracle & 65.96 & 39.86 & 58.60 & 31.08 & 89.02 & 82.93 & 32.82 & 88.62 & 79.10 \\
        \midrule
        \multirow[c]{4}{*}{Mistral-Ins V0.3} & CodeRM & \bfseries 34.04 & \bfseries 7.43 & \bfseries 27.54 & \bfseries 7.43 & \bfseries 61.59 & \bfseries 53.05 & nan & \bfseries 58.99 & \bfseries 49.74 \\
        & average & 20.33 & 4.10 & 16.04 & 2.70 & 37.04 & 30.95 & nan & 44.59 & 37.78 \\
        & greedy & 25.88 & 6.08 & 20.09 & 5.41 & 36.59 & 31.10 & nan & 49.47 & 41.27 \\
        & oracle & 52.72 & 25.68 & 44.04 & 18.92 & 75.00 & 68.90 & nan & 75.93 & 65.61 \\
        \midrule
        \multirow[c]{4}{*}{Qwen-Coder-2.5} & CodeRM & \bfseries 50.18 & \bfseries 27.70 & \bfseries 44.91 & \bfseries 22.97 & 90.85 & 85.37 & \bfseries 38.29 & \bfseries 85.19 & \bfseries 72.22 \\
        & average & 42.69 & 16.34 & 37.75 & 14.95 & 85.21 & 79.23 & 31.74 & 77.60 & 64.83 \\
        & greedy & 49.47 & 19.59 & 41.84 & 20.27 & \bfseries 91.46 & \bfseries 85.98 & 34.19 & 82.80 & 71.43 \\
        & oracle & 69.74 & 50.00 & 66.40 & 41.22 & 96.34 & 92.68 & 51.47 & 96.03 & 87.30 \\
        \bottomrule
        \end{tabular}
        }
\end{table*}


\begin{table*}[!tbh]
\centering
    \caption{CodeRM's best-of-n results. We evaluated the model on MBPP, HumanEval (HE), BigCodeBench (BCB), and LiveCodeBench (LCB). Specifically, we have evaluated the Completion (C) and Instruct (I) splits of BCB for both Hard (H) and Full (F) versions, and also the plus version for MBPP and HE.}
    \label{tab:wide-table}
    \small
    \resizebox{\textwidth}{!}{
        \begin{tabular}{ccclllllllll}
            \toprule
            \multirow{2}{*}{Policy Model} & \multirow{2}{*}{Method} & \multirow{2}{*}{\# N} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{MBPP} & \multicolumn{2}{c}{BigCode (C)} & \multicolumn{2}{c}{BigCode (I)} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}LiveCode\\ V4\end{tabular}} \\
             &  &  & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Plus} & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Plus} & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{Hard} & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{Hard} &  \\
             \midrule
            \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}CodeLlama\\ -Ins-7B\end{tabular}} & Greedy & 1 &  &  &  &  &  &  &  &  &  \\
             & Random & 64 &  &  &  &  &  &  &  &  &  \\
             & Oracle & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 64 &  &  &  &  &  &  &  &  &  \\
             \midrule
            \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Llama-3.1\\ -Ins-8B\end{tabular}} & Greedy & 1 &  &  &  &  &  &  &  &  &  \\
             & Random & 64 &  &  &  &  &  &  &  &  &  \\
             & Oracle & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 64 &  &  &  &  &  &  &  &  &  \\
             \midrule
            \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Mistral\\ -Ins-V0.3-7B\end{tabular}} & Greedy & 1 &  &  &  &  &  &  &  &  &  \\
             & Random & 64 &  &  &  &  &  &  &  &  &  \\
             & Oracle & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 64 &  &  &  &  &  &  &  &  &  \\
             \midrule
            \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Qwen\\ -Coder-2.5-7B\end{tabular}} & Greedy & 1 &  &  &  &  &  &  &  &  &  \\
             & Random & 64 &  &  &  &  &  &  &  &  &  \\
             & Oracle & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-7B & 64 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 16 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 32 &  &  &  &  &  &  &  &  &  \\
             & CodeRM-32B & 64 &  &  &  &  &  &  &  &  &  \\
             \bottomrule
            \end{tabular}
     }
\end{table*}



